You Can Do Better! If You Elaborate the Reason When Making Prediction

Neural predictive models have achieved remarkable performance improvements in various natural language processing tasks. However, most neural predictive models suffer from the lack of explainability of predictions, limiting their practical utility. This paper proposes a neural predictive approach to make a prediction and generate its corresponding explanation simultaneously. It leverages the knowledge entailed in explanations as an additional distillation signal for more efficient learning. We conduct a preliminary study on Chinese medical multiple-choice question answering, English natural language inference, and commonsense question answering tasks. The experimental results show that the proposed approach can generate reasonable explanations for its predictions even with a small-scale training corpus. The proposed method also achieves improved prediction accuracy on three datasets, which indicates that making predictions can benefit from generating the explanation in the decision process.

==> impact.tex <==
\section{Broader Impact}
Our research primarily deals with deploying high quality NLP applications to a wide audience around the globe. We contend that these technologies can simplify many of our mundane tasks and free up our time to pursue more pleasurable work. We are well aware that in themselves they are no panacea and any time that they free up may well be exploited by the very companies which distribute these for profit. However, we try to be humble and solve the problem at hand and encourage all the stakeholders to play their part.
